2D Gaussian Splatting for Geometrically Accurate Radiance Fields

3D Gaussian Splatting (3DGS) has recently revolutionized radiance field reconstruction, achieving high quality novel view synthesis and fast rendering speed without baking. However, 3DGS fails to accurately represent surfaces due to the multi-view inconsistent nature of 3D Gaussians. We present 2D Gaussian Splatting (2DGS), a novel approach to model and reconstruct geometrically accurate radiance fields from multi-view images. Our key idea is to collapse the 3D volume into a set of 2D oriented planar Gaussian disks. Unlike 3D Gaussians, 2D Gaussians provide view-consistent geometry while modeling surfaces intrinsically. To accurately recover thin surfaces and achieve stable optimization, we introduce a perspective-correct 2D splatting process utilizing ray-splat intersection and rasterization. Additionally, we incorporate depth distortion and normal consistency terms to further enhance the quality of the reconstructions. We demonstrate that our differentiable renderer allows for noise-free and detailed geometry reconstruction while maintaining competitive appearance quality, fast training speed, and real-time rendering.

==> tables/algorithm.tex <==
\begin{algorithm}
\caption{2D Gaussian Splatting Algorithm \\
$\bp, s_u, s_v$: center, two scaling factors\\
$\bu,\bv$: two tangent vectors\\
$\bc, \alpha$: color and opacity \\
$\bM, \bP$: viewing matrix and projection matrix
}
\begin{algorithmic}

\Function{RasterizationSetup}{$p$, $s_u$, $s_v$, $\bt_u$, $\bt_v$}
% \State \textbf{Rasterization Setup:}
    \State $T \gets 
    \begin{pmatrix} 
    s_u\bt_u & s_v\bt_v & \mathrm{0} & \bp \\
    0 & 0 & 0 & 1 
    \end{pmatrix}$ 
    \State $T \gets {(PMT)}^\top$
    \State $d \gets (\{1, 1, -1\}, (T_4 \cdot T_4))$ \Comment{Viewing transform}
    \State $f \gets (\{1, 1, -1\})$
    \State $p_i \gets (f, (T_i \cdot T_4))$
    \State $h_i \gets \sqrt{p_i^2} - (f, (T_i \cdot T_i))$ \Comment{Bounding Box}
\EndFunction

\State
\Function{Rasterization}{$T$}
\State $w(x,y) \in \{h_i^x, h_i^y, c_i^x + h_i^y\}$
\State $k \gets -T_1 + xT_4$
\State $l \gets -T_2 + yT_4$
\State $s \gets (l_4(k,l), l_2(k,l))$
\State $\rho^2 \gets (s, (s/r - (k/l_2 - h_i)^2))$
\EndFunction
% \State $\rho^2 \leq \text{cutoff}^2 \ ? \ \text{inside} : \text{outside, kill}$
% \State $w_f \gets k(\rho^2)$

\end{algorithmic}
\end{algorithm}


==> tables/nerf.tex <==
\begin{table}[t]
\centering
\label{tab:nerf_synthetic}
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|ccccccccc}
 & \textbf{Mic} & \textbf{Chair} & \textbf{Ship} & \textbf{Materials} & \textbf{Lego} & \textbf{Drums} & \textbf{Ficus} & \textbf{Hotdog} & \textbf{Avg.} \\
\hline
Plenoxels   & 33.26 & 33.98 & 29.62 & 29.14 & 34.10 & 25.35 & 31.83 & 36.81 & 31.76 \\
INGP-Base   & 36.22 & 35.00 & 31.10 & 29.78 & 36.39 & 26.02 & 33.51 & 37.40 & 33.18 \\
Mip-NeRF    & 36.51 & 35.14 & 30.41 & 30.71 & 35.70 & 25.48 & 33.29 & 37.48 & 33.09 \\
Point-NeRF  & 35.95 & 35.40 & 30.97 & 29.61 & 35.04 & 26.06 & 36.13 & 37.30 & 33.30 \\
3DGS        & 35.36 & 35.83 & 30.80 & 30.00 & 35.78 & 26.15 & 34.87 & 37.72 & 33.32 \\
2DGS~(Ours)        & 35.09 & 35.05 & 30.60 & 29.74 & 35.10 & 26.05 & 35.57 & 37.36 & 33.07 \\
\end{tabular}
}
\label{tab:nerf}
\caption{PSNR scores for Synthetic NeRF. Our 2D Gaussian Splatting is comparable to the state-of-the-art methods on novel view synthesis even without regularizations.}
\end{table}
